An unsupervised method for identifying $X$-enriched stars directly from spectra: Li in LAMOST

Stars with peculiar element abundances are important markers of chemical enrichment mechanisms. We present a simple method, tangent space projection (TSP), for the detection of $X$-enriched stars, for arbitrary elements $X$, even from blended lines. Our method does not require stellar labels, but instead directly estimates the counterfactual unrenriched spectrum from other unlabelled spectra. As a case study, we apply this method to the $6708~$\AA{} Li doublet in LAMOST DR5, identifying 8,428 Li-enriched stars seamlessly across evolutionary state. We comment on the explanation for Li-enrichement for different subpopulations, including planet accretion, nonstandard mixing, and youth.

==> random_30000_test.classified.tex <==
\tablehead{\colhead{\texttt{obsid}} & \colhead{\texttt{best\_fit\_chi2}} & \colhead{\texttt{isline}} & \colhead{\texttt{amplitude}} & \colhead{\texttt{delta\_chi2}}}
\startdata
101034 & 4982.8853 & True & -0.0271 & 0.3953 \\
101040 & 2341.6377 & True & -0.0899 & 0.8633 \\
101056 & 3257.179 & True & -0.0942 & 1.5961 \\
101061 & 3513.186 & True & -0.0485 & 1.6001 \\
101092 & 3021.3784 & True & -0.053 & 10.1769 \\
101171 & 4519.6357 & False & -0.0041 & nan \\
101175 & 3989.1453 & True & -0.0262 & 0.2298 \\
102038 & 2945.8486 & False & 0.0224 & nan \\
102108 & 2811.592 & False & 0.0029 & nan
\enddata
